Scaling Down Text Encoders of Text-to-Image Diffusion Models

Text encoders in diffusion models have rapidly evolved, transitioning from CLIP to T5-XXL. Although this evolution has significantly enhanced the models' ability to understand complex prompts and generate text, it also leads to a substantial increase in the number of parameters. Despite T5 series encoders being trained on the C4 natural language corpus, which includes a significant amount of non-visual data, diffusion models with T5 encoder do not respond to those non-visual prompts, indicating redundancy in representational power. Therefore, it raises an important question: "Do we really need such a large text encoder?" In pursuit of an answer, we employ vision-based knowledge distillation to train a series of T5 encoder models. To fully inherit its capabilities, we constructed our dataset based on three criteria: image quality, semantic understanding, and text-rendering. Our results demonstrate the scaling down pattern that the distilled T5-base model can generate images of comparable quality to those produced by T5-XXL, while being 50 times smaller in size. This reduction in model size significantly lowers the GPU requirements for running state-of-the-art models such as FLUX and SD3, making high-quality text-to-image generation more accessible.

==> table/size_vs_performance.tex <==

\begin{table*}[t]
\vspace{5pt}
\centering
\small 
\resizebox{\linewidth}{!}{
\begin{tabular} {l  c  c c  c c c c c c  c c c }
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Size}}}  
  & \multicolumn{2}{c}{\textbf{Aesthetics}}      
  & \multicolumn{6}{c}{\textbf{Composition}}     
  & \multicolumn{3}{c}{\textbf{Text Rendering}} \\
              \cmidrule(lr){3-4} \cmidrule(lr){5-10} \cmidrule(lr){11-13}
 \multicolumn{2}{c}{}  & FID~($\downarrow$) & CLIP-Score~($\uparrow$) & Color~($\uparrow$) & Shape~($\uparrow$) & Texture~($\uparrow$) & 2d-spatial~($\uparrow$) & 3d-spatial~($\uparrow$) & Numeracy~($\uparrow$) & Character~($\uparrow$) & Word~($\uparrow$) & Sentence~($\uparrow$) \\
\midrule 
T5-Small & 60 M & 25.10 & 28.28 & 72.55 & 39.62 & 60.23 & 25.28 & 40.89 & 53.51 & 31.91 & 12.01 & 9.3 \\ 
    T5-Base & 220 M & 24.32 & 29.79 & 73.41 & 43.54 & 63.96 & 25.52 & 40.18 & 55.28 & 69.30 & 42.42 & 35.6  \\ 
T5-Large & 770 M & 24.19 & 29.89 & 74.86 & 51.08 & 64.96 & 24.79 & 39.86 & 56.62 & 69.52 & 43.76 & 36.3 \\
T5-XL  & 3,000 M & 23.17 & 30.33 & 77.83 & 54.86 & 66.37 & 24.94 & 40.40 & 58.43 & 77.76 & 57.67 & 48.8  \\

\midrule 
T5-xxl~(teacher) & 12,000 M & 22.36 & 31.30 & 79.11 & 57.22 & 68.88 & 27.24 & 39.84 & 61.08 & 76.79 & 59.29 & 51.2 \\ 
\bottomrule
\end{tabular}

}
\caption{
\label{table:different_t5}
{\bf Model size vs. performance.} We trained a series of T5 encoder models using the same data and procedures. We tested their performance comprehensively in three aspects: aesthetics, composition, and text rendering.
}
\end{table*}


        
